Rational Ponzi Games in Algorithmic Stablecoin

Algorithmic stablecoins (AS) are one special type of stablecoins that are not backed by any asset (equiv. without collateral). They stand to revolutionize the way a sovereign fiat operates. As implemented, these coins are poorly stabilized in most cases, easily deviating from the price target or even falling into a catastrophic collapse (a.k.a. Death spiral), and are as a result dismissed as a Ponzi scheme. However, is this the whole picture? In this paper, we try to reveal the truth and clarify such a deceptive concept. We find that Ponzi is basically a financial protocol that pays existing investors with funds collected from new ones. Running a Ponzi, however, does not necessarily imply that any participant is in any sense losing out, as long as the game can be perpetually rolled over. Economists call such realization as a \textit{rational Ponzi game}. We thereby propose a rational model in the context of AS and draw its holding conditions. We apply the model to examine: \textit{whether or not the algorithmic stablecoin is a rational Ponzi game.} Accordingly, we discuss two types of algorithmic stablecoins (\text{Rebase} \& \text{Seigniorage shares}) and dig into the historical market performance of two impactful projects (\text{Ampleforth} \& \text{TerraUSD}, respectively) to demonstrate the effectiveness of our model.

==> Section/1intro.tex <==
\section{Introduction}
\label{sec:intro}
Ponzi is making a comeback that is used to describe the hyped algorithmic stablecoins today. The most recent critique was directed at the one called TerraUSD (UST), which crashed by almost 98\% within 24 hours on May 12$^{\text{th}}$, 2022 (cf.\cite{coinmarketcap}), impacting a direct of \$85B market value evaporation and the collapse of entire crypto markets. This worst-hit reveals a new type of bank run and has triggered repetitive rounds of criticism and discussion about the stablecoin and its algorithmic stabilized approaches. Stablecoins are created to share all great features that cryptocurrencies hold (e.g., decentralization, automation, cross-border), without, however, suffering from the same volatility, making them much more applicable as a store of value, medium of exchange, and unit of account~\cite{sokemin,stablecoins2.0,demys_stable}.
In an ideal form, stablecoins are simply cryptocurrencies with stable value. Current stablecoin implementations (cf. Tab.\ref{tab:stablecoin}) aim to bridge external assets with the cryptocurrency space by anchoring a peg (e.g., USD) in price. 

\input{table/stablecoins}


Stablecoins in cryptocurrencies are generally tagged as either collateralized or algorithmic stablecoins in terms of their specific collaterals. The collateralized stablecoin, as the name implies, requires collateral and thus ensures the circulating token having a redemption value. Possible collateral options include fiat money, cryptocurrency, and other valuable assets.
Currently, stablecoins are majorly backed by fiat money (Tab.\ref{tab:stablecoin}). USDC \cite{usdc}, for example, is a fully collateralized stablecoin pegged to USD and stores its US dollars in a number of banks. Such a type of stablecoins, backed by fiat money, are generally of a high degree of centralization. Instead, using cryptocurrencies as collateral can circumvent this problem. However, considering the high volatility, an \textit{over}-collateralization is thereby required if relying on cryptocurrencies as collateral.  One representative in this category is the stablecoin DAI \cite{dai}, where a user needs to deposit Ether (the native token of Ethereum) in excess of the amount of created DAIs. Even if the collateral crypto depreciates, each unit of the stablecoin still has enough space of being redeemed for at least an equivalent amount of underlying assets.


Algorithmic stablecoin (AS), however, does \textit{not} require any collateral. The money supply of algorithmic stablecoin is elastic and managed by algorithms (i.e., coded in smart contracts). Algorithmic stablecoins are thus not limited in scale by the circulating amount of the underlying collateral. For stabilization, the par value of an algorithmic stablecoin is basically preserved by expanding supply when the price is too high and contracting it when the price is too low. Two distinct AS designs are prevailing in markets \cite{volatility}, namely, \textit{rebase} and \textit{seigniorage shares}. 
Rebase~\cite{hayekrebase} is an algorithm that automatically adjusts the money supply in response to the market demand on a routine basis. A rebase protocol can add (\texttt{mint}) or remove (\texttt{burn}) coins from circulation according to the stablecoin's price deviation from the peg, and this is normally achieved by adjusting token balance pro rata across all wallets. Instead of rebasing one coin, seigniorage shares~\cite{noteonshares} normally has a \textit{dual} (or \textit{multiple}) coin design: the price-stable coins and flexible investment shares. The shares algorithmically expand and contract the supply of price-stable coins much like a central bank does with fiat currencies. Seigniorage shares model has, to varying degrees, served as a foundation for TerraUSD \cite{TerraUSD}, Empty Set \cite{emptyset}, Basis Cash \cite{basiscash}, and Frax \cite{frax}.

\smallskip
\noindent\textbf{Contributions.} Unfortunately, no satisfactory algorithmic stablecoins have been healthily operated for a long-term run. Non-stable performance and non-collateral property destroy the natural trust of participants and communities. AS schemes are thus often questioned as Ponzi schemes. This motivates our observations towards this fancy but fuzzy concept. \textit{\text{First}}, we comprehensively review existing in-the-wild AS projects and 
explore the design primitives they share in common (Sec.\ref{sec:intro}). \textit{\text{Then}}, we accordingly have established a rational Ponzi model in the context of algorithmic stablecoins (Sec.\ref{sec:model}) and \textit{\text{further}} evaluate two mainstream projects, namely, Ampleforth and TerraUSD (the representatives of \text{Rebase} and \text{Seigniorage share}, respectively), based on six-month historical data from Mar 1$^\text{st}$ to Oct 17$^\text{th}$ 2022 (Sec.\ref{sec:apply}). \textit{\text{Also}}, we find several interesting insights (Sec.\ref{sec:discuss}) that are driven by our model. \textit{\text{Last}}, we deliver a taking-home message saying: \textit{the rebase approach is much more likely to achieve a rational Ponzi game as long as it always exists in an active trading market whereas the seigniorage share method is, if without external interruptions, of low probability to realize it due to the uncontrollable death spirals from the overlapped effect of dual coins}.




\smallskip
\noindent\textbf{Recent Studies.} 
A series of papers and reports~\cite{demys_stable,designstablecoins,stablecoinsurvey,multicoinsry} establish and extend the taxonomies in stablecoins based on the peg type, the collateral type, and the collateral amount. They give an initial sight to demystify its assemblies and components. Besides, with in-depth analysis, a bunch of follow-up works is proposed.  Moin et al. \cite{sokemin} provide a systematical classification of existing stablecoins in terms of their design elements.  Ariah et al. \cite{stablecoins2.0} explore the economic structure of stablecoins and establish a risk-based functional characterization. Pernice et al. \cite{openquestion} research stablecoins from a monetary perspective. Salehi et al. \cite{dai_liquidation} explore the liquidation process in stablecoins, and put forward a research agenda for alternatives to liquidation. Clements R. \cite{clements2021builttofail} studies the inherent fragility in algorithmic stablecoins and claims that they are built to fail. Zhao et al. \cite{volatility} conduct an empirical analysis to explain the volatility of algorithmic stablecoins.



% A paper by Pernice et. al takes a different approach, categorizing stablecoins by monetary and exchange rate regimes [53].

% Studies investigating the asset class and its manifestations include [cite] and [cite].
% The user perception in the adoption of stablecoins has been studied in [], while [] analyzed the suitability of stablecoins as save-haven investment.
% The relation between cryptocurrency prices and stablecoin trading has been focused on by [] and []. 
% Adopting a risk-oriented approach, [] and [] suggest theoretic models to study stability and resilience of stablecoins. While the latter focuses on extreme events, [] not only offers a theoretic model for day-to-day arbitrage but also provides, to my knowledge, the first extensive empirical analysis of the drivers of stablecoin prices. 



% \begin{wraptable}{r}{5cm}
%  \caption{Stablecoin Category} 
%  \label{tab:stablecoin}
%   \centering
%  \resizebox{\linewidth}{!}{ \begin{tabular}{l r}
%     \toprule
%       & \textbf{Collateral Type}  \\
%     \midrule
%     \multirow{3}{*}{\textit{Collateral}}  &  Fiat collateral  \\
%       &  Crypto collateral  \\
%       &  Other collateral  \\
%     \cmidrule{1-2}
%     \textit{Partial-collateral}  & - \\ 
%     \cmidrule{1-2}
%     \multirow{2}{*}{\textit{\makecell{Algorithmic \\(non-collateral)}}} & \cellcolor{pink} Rebase \\
%     &  \cellcolor{pink} Seigniorage shares \\
%     \bottomrule
%   \end{tabular}}
%   \label{server}
% \end{wraptable}
% % blue!25



% https://drive.google.com/file/d/1BADClaZBZhXkYdsMxaJ6icJhNFlWuvV9/view?usp=sharing


% However, the cryptocurrency collateral itself is highly volatile,
% compared to fiat currency,
% thus making it hard to use as a guarantee of value.
% Crypto collateral are managed by smart contract, a self-executing program, thus eliminating the dependence on a third party.
% Specifically, collateral deposit can be accessed by paying back the stablecoin debt, or can be automatically liquidated if the value of collateral falls below a certain threshold.






% \noindent\textbf{Roadmap.} 
% The roadmap of this work is as follows.
% We briefly review related works in Section~\ref{sec:relatedwork}.
% % In Section~\ref{sec:background}, we break down the taxonomy of stablecoins as collateral stablecoin and algorithmic stablecoin (i.e., without collateral, abbreviated as AS).
% % In Section~\ref{sec:background}, we investigate the classification of algorithmic stablecoin (i.e., without collateral, abbreviated as AS) and their corresponding mechanics.
% In Section~\ref{sec:model}, we construct a concise model of rational Ponzi game.
% We then examine whether Ampleforth (rebase) and TerraUSD (Seigniorage Shares) meet the conditions of being rational Ponzi games.
% Finally, we provide conclusion remarks in Section~\ref{sec:conclusion}.




==> Section/2model.tex <==
\section{Modeling Rational Ponzi Games}
\label{sec:model}

Ponzi~\cite{ponzi_wiki} has always been such a term that is instinctively resented by the public. For malicious organizers, Ponzi schemes are used to lure new investors, and leverage incoming money to pay earlier ones while keeping the rest as profit.
In general, organizers will promise an abnormally high return to investors within the short term. With little or no legitimate earnings, Ponzi games require a constant flow of new funds to survive. Once becoming difficult to recruit new participants, or whenever a large number of existing investors cash out, these games tend to collapse. 
However, stemming from its origin, the substance of Ponzi is neutral yet subtle. Economists~\cite{ponzi_minsky,ponzi_kindleberger} discuss a perfect foresight version of the Ponzi model, where the schemes based on imperfect information or irrationality of lenders are ruled out. They call such a policy, in which all repayments are forever \textit{rolled over}, i.e., financed by issuing new debt, a \textit{rational Ponzi game}~\cite{ponzi_rational}. Following such narrative connotations, we develop the model in the context of algorithmic stablecoins. 


% By engaging in a Ponzi game, the borrower is able to extract positive resources (in present value terms) from the lender(s). The classic form of this scheme consists of borrowing money (issuing short or long term debt) and financing all promised payments of principal or interest by issuing new debt. 

% sequence

\smallskip
\noindent\textbf{Rational Ponzi Game.}
An entity that plans to issue debt and roll it over the possibly infinite future is the borrowing side of a rational Ponzi game. Any plan will impose a set of net cash inflows $I_s$ from the lending side. The present value of borrower's net indebtedness $D_{T}$ of at any time $T$ equals the present value of the stream of prospective incomes generated by lenders between $0$ and $T$:

\begin{equation}
\Gamma(T) D_{T}=\sum_{s=1}^{T} \Gamma(s) I_{s}
\end{equation}
where $\Gamma(T)$ is the discount factor of the borrowing side, it is calculated by the interest rate $r_{t}$ between periods $t-1$ and $t$\footnote{In corporate finance, a discount factor is a number that is derived from the discount rate. It is used to discount future cash flows back to their present value at a specific discount rate. Here, we assume $r_{t}$ are identical for all assets under perfect foresight.}, and $\Gamma(s)$ is the discount factor applicable in period 0 to cash inflows received in the period $s$, where
$ \Gamma(s) \equiv \prod_{j=1}^{s}\left(1+r_{j}\right)^{-1}.$ 
We now provide the definition of a rational Ponzi game.

\begin{defi}[Rational Ponzi Game]\label{defi-ponzi}
A rational Ponzi game is a sequence of debt transactions satisfying the following sense: \begin{itemize}
    \item[(i)] to the borrower, it is a positive net present indebtedness value such that $\lim _{T \rightarrow \infty}$ $\Gamma(T) D_T>0$, if the limit of $\Gamma(T) D_T$ exists;
    \item[(ii)] to all the participants, i.e., both the borrowing and lending sides, the game enables a Pareto improvement\footnote{A Pareto improvement is an improvement to a given situation, where a change in allocation of goods harms no one and benefits at least one individual.}.
\end{itemize}
\end{defi}

The first holding condition in Definition 1 implies that debts 
are unnecessarily fully paid off by future cash inflows if in an infinite horizon setting. The second condition imposes restrictions that no one is being worse (assets can always be redeemed at least equal to the market value of assets deposited). Therefore, the two conditions guarantee a rational realization. We provide a general operation process of rational Ponzi schemes as in Fig~\ref{fig:rational}. The red plus sign and the green minus sign represent cash inflow and cash outflow, respectively. The values in parentheses following each participant represent their corresponding utility.


%you can edit the figure here: https://drive.google.com/file/d/1yK-DRCSBQIFNEzGlQW87cfWnQ03dqLj7/view?usp=sharing

\begin{figure}[H]
	\centering
	\includegraphics[scale=0.56]{figs/rational_ponzi_demo.pdf}
	\vspace{-0.3cm}
	\caption{A general flow interpreting how a rational Ponzi game works.} 
	\label{fig:rational}
 	\vspace{-0.5cm} 
\end{figure}

\noindent\textbf{Scope of application.} One may consider that only governments are entitled to run such rational Ponzi games. However, in a world where rational Ponzi games can exist, any infinitely lived entity can issue debt and perpetually roll it over. In principle, even a finitely lived entity can issue bonds with zero coupon, i.e., fiat money. All required is to make participants believe that there will always exist followers being willing to purchase the debt. Meanwhile, economists have proven that the introduction of perpetually rolled over debt will never make the lending economy worse off relative to a world in which no Ponzi game runs~\cite{ponzi_rational,tirole1985asset,pernice2019monetary}.




\section{Applied to Algorithmic Stablecoins}
\label{sec:apply}

Typically, algorithmic stablecoins, based on their operating mechanisms, can be considered a Ponzi game: an on-chain protocol launches a coin (equiv. debt) claimed to be stable (investors can always obtain the equivalent fund back when selling the coin), and one joins the game by purchasing the coin and can quit the game if others are willing to buy his coins on the market. However, is such an algorithmic stablecoin game \textit{rational} under our model? In this section, we instigate two typical instances, Ampleforth (rebase) and TerraUSD (seigniorage shares), to answer this question.
Supposing that all the lending protocols are deployed on smart contracts on a public ledger so that all steps are perfectly enforceable (equiv. no default risk). We define the notation $\mathcal{U}$ as the investor's utility; it is basically the product of the number of held assets $Q$ and the market price of the token $P$, in symbols as
\begin{equation}
\mathcal{U} = Q \times P.
\end{equation}

Then, we apply our model to two concrete instances by investigating their six-month historical data (Mar\,--\,Oct, 2022). We analyze the utility of investors based on extracted data covering price, quantity, and market cap.

\smallskip
\noindent\textbf{Ampleforth.} 
Ampleforth (AMPL) \cite{ampleforth} is an algorithmic stablecoin protocol that applies the design of rebase. AMPL is pegged to the CPI-adjusted USD, and its rebase procedure occurs at 02:00 UTC on a daily basis. The quantity of AMPL tokens in user accounts automatically expands or contracts based on everyday price.
% The rebase() method first queries the Market Oracle to get the current price. If the price is within priceThreshold of the target price, no supply policy change is applied.
%
According to Ampleforth white paper~\cite{amplwhiterpaper}, the absolute \texttt{supplyDelta} of AMPL is equal to \texttt{(price-target)*totalSupply/target}.
For example, at the time of rebase, if the price of AMPL is \$1.1, 10\% greater than the standard 1 USD peg, a wallet with a balance of 100 AMPL will be rebased as 110 accordingly. In contrast, when the AMPL price is less than 1 USD, the protocol will proportionally decrease the quantity of tokens in wallets, aiming to bring the price up to its anchor.


\begin{figure}[!hbt]
	\centering
	\includegraphics[width=1\textwidth]{figs/ampf.png}
	\caption{AMPL price, number of AMPL, and investor's utility over time.}
	\label{fig:ampl}
\vspace{-0.4cm}
\end{figure}


\smallskip
\noindent\textit{Investor's utility analysis.}
Considering an investor who participates in the Ampleforth game at any time by purchasing one unit of AMPL, we analyze the changes in his utility over time. At each rebase time (cf. Fig.\ref{fig:ampl}), the investor's utility (red line) stays the same\footnote{Except for the rebase time in a day, the number of AMPL in wallets will not change. If the coin price rises and the investor selects to sell, his utility is greater than his original investment.}, meaning that the investor can always redeem (trade) the identical value of his investment back. However, the price of AMPL (green line) cannot keep stable, and the AMPL balance (blue line)\footnote{To better demonstrate the nature of rebase, we calculate daily AMPL numbers based on a simple settings from its 1st version whitepaper~\cite{amplwhiterpaper}.} is in the investor's wallet. In terms of a rational Ponzi model, AMPL has the potential to satisfy all listed conditions as long as there exists an lively traded market. 

Since any investor can retain at least the same utility in the AMPL network, regardless of the price of the token, one may wonder why the rebase is not being adopted on a larger scale. The most obvious reason is due to its highly volatile price, resulting in holding AMPL being no different than holding a regular cryptocurrency. At the same time, one's balance varies proportionally to the price every day, making the holder fall into passive and anxious emotions. Besides, AMPL, as an ERC-20 token that works natively on Ethereum blockchain, cannot perform its rebase implementation smoothly in a centralized exchange or other blockchain platforms, significantly restricting its use scenarios. Ampleforth mitigates this constraint with the release of Wrapped-AMPL, a token that wraps AMPL similar to wrapped ETH. Wrapped-AMPL facilitates ecosystem integrations on both centralized and decentralized platforms. 


\smallskip
\noindent\textbf{TerraUSD.} 
TerraUSD (UST) \cite{TerraUSD} is a seiniorage shares style stablecoin pegging to the USD on top of Terra's blockchain. LUNA, as the native staking token of the Terra blockchain, absorbs the volatility from UST.
Aibitrage can help making UST price stable: when the UST's price is $<1$ USD, arbitragers can send 1 UST to the system and receive 1 USD's worth of LUNA; whereas the UST's price becomes $>1$ USD, arbitragers will send 1 USD's worth of LUNA to the system and receive 1 UST.

\begin{figure}[!hbt]
	\centering
	\includegraphics[width=1\textwidth]{figs/ust.png}
	\caption{UST price, number of UST, and investor's utility over time.} 
	\label{fig:ust}
	\vspace{-0.3cm}
\end{figure}


\noindent\textit{Investor's utility analysis.}
We also consider an investor who participates in the UST game at any time by purchasing one unit of UST. For simplicity, we assume that the investor will always hold UST without converting him to LUNA in the mid-run before exiting the game.  A chart of UST price (green line), the number of UST in the wallet (red line), and the investor's utility (blue line) over time are presented in Fig.\ref{fig:ust}.
The practice proves the ineffectiveness of UST's stabilization as the UST eventually collapsed.
Investors suffered a significant loss from their initial investments,
% even though the token claimed its value could stay stable.
making UST unlikely to become a rational Ponzi game.
% We here examine the reasons that result in such failure by finding the unsatisfied requirements defined in our rational model.

In fact, current designs of seigniorage shares are practically difficult for realizing a rational model. These stablecoins are not substantially secured by anything, other than the expectation that the stablecoin will eventually appreciate in value. Hence, a necessary condition for the seigniorage shares to work healthy is that the secondary coin has to have values. LUNA, as the secondary coin, should have, at least, trading values, as people do use Terra blockchain every day. However, in extreme cases, investors may still lose confidence in it, and the massive sell-off has accelerated both two types of coins into a death spiral faster.


% non-pegged coin: 
% death spriral is the key why not achieve rational to such design.
% If there is a malicious actor intent on sabotaging the stability,
% 3 cases: price up, flat, down.

% As long as people are using the Terra/Luna blockchain, Terra should retain some value.
% Fees and rewards, also paid in Luna, are additionally adjusted to entice users to buy and hold Luna even during downturns.




==> Section/3discuss.tex <==
\section{Discussion}
\label{sec:discuss}

\noindent\textbf{Market cap vs price stability.}
The investors involved in stablecoin markets often have intuitive feelings that the larger the market cap of the stablecoin, the better stability the stablecoin can achieve with regard to its peg. However, according to the price and market cap data from CoinGecko \cite{coingecko}, this conjecture may not be valid as imagined for algorithmic stablecoins. The statement of ineffective application to the rebase design is explicit, as its market capitalization will vary as the supply of the currency is adjusted. For the seigniorage share design, this statement will be invalid as well. Due to its relative complexity, there are a lot of possibilities resulting in this situation, one of which is the loss of confidence. The recent joint collapse of LUNA/UST was a loop in which the market lost confidence and entered a death spiral, pushing them out of the market cap top 10 within merely several hours. Thus, a larger market cap in algorithmic stablecoin does not necessarily guarantee better stability.


\smallskip
\noindent\textbf{Price oracle risk.}
Price oracle provides the price feed for on-chain DeFi protocols \cite{werner2021sok}, and it is crucial to the secure operation of an algorithmic stablecoin. Algorithmic stablecoins may have special price-feeding needs due to the existence of algorithms, which further need to establish their own oracles. An internal oracle, however, will inevitably lead to an additional layer with potential centralization and incentivize the coin issuer to update the price in his favor. In contrast, opting for an external price oracle may mitigate this problem, but it is still vulnerable to external price manipulation, being out of the control of the coin issuer. Relevant attacks include flash loan price manipulation attack, pump, and dump~\cite{Attackflashloan}. Selecting a trustworthy price oracle is not easy for an algorithmic stablecoin, and a comprehensive ex-ante risk assessment is required.

\smallskip
\noindent\textbf{Reconsider the necessity of a peg.}
Stablecoins are designed to be pegged to some underlying assets, with the USD being a popular choice. Anchoring a benchmark is an effective way to achieve stability in stablecoins. People may thus generally assume a fact that the stablecoin is perfectly fungible for its peg. However, this is not the full truth. Stablecoins can be, in fact, rather considered as their own free-floating assets that closely track the value of a peg. Besides, it is also possible that stablecoins could provide the desired stability without pegging to an asset. In one possible future, once the economy develops surrounding the stablecoin itself, and such stablecoins have also been widely used as a medium of exchange, maintaining a perfect peg becomes unnecessary.




% \begin{figure}[!hbt]
% 	\centering
% 	\includegraphics[width=1\textwidth]{figs/marketcap.png}
% 	\caption{Market Cap and Utility.} 
% 	\label{fig:marketcap}
% \end{figure}


==> Section/4conclude.tex <==
\section{Concluding Remarks}\label{sec:conclu}
% This study creatively applies O'Connell \& Zeldes's model (1988, cf.\cite{ponzi_rational}) to the context of algorithmic stablecoins.
% Following its connotation, we establish a rational Ponzi game as the measurement and accordingly evaluate two mainstream algorithmic stablecoin projects (Ampleforth and TerraUSD) as instances.

This study creatively applies O'Connell \& Zeldes's model (1988, cf.\cite{ponzi_rational}) for rational Ponzi games to the context of algorithmic stablecoins. Our analyses of investors' utilities indicate that the rebase approach has the potential to realize a rational Ponzi game as long as it always exists in an active trading market. Notably, by leveraging smart contracts, DeFi protocols will be much easier to realize a rational Ponzi model than those in centralized finance, by means of many advanced and innovative financial tools like automated market makers (AMM), flash loans, and enforceable payment. In contrast, the seigniorage share method is difficult to guarantee a rational Ponzi, as dealing with the selling pressure in a death spiral for dual coins is intrinsically complicated. Beyond that, we point out the hurdles existing in current algorithmic stablecoin implementations and further identify the potential opportunities for future endeavors. 
% To the best of our knowledge, this paper proposes the first study for identifying, establishing, deciding, and evaluating rational Ponzi games in the track of algorithmic stablecoins. 


% and put forward a research agenda for alternatives to ration model in algorithmic stabecoins.



==> Section/5releatedwork.tex <==
\section{Related Works}
\label{sec:related}
% \noindent\textbf{Recent Studies.} 
A series of papers and reports~\cite{demys_stable,designstablecoins,stablecoinsurvey,multicoinsry} establish and extend the taxonomies in stablecoins based on the peg type, the collateral type, and the collateral amount. They give an initial sight to demystify its assemblies and components. Besides, with in-depth analysis, a bunch of follow-up works is proposed.  Moin et al. \cite{sokemin} provide a systematical classification of existing stablecoins in terms of their design elements.  Ariah et al. \cite{stablecoins2.0} explore the economic structure of stablecoins and establish a risk-based functional characterization. Pernice et al. \cite{openquestion} research stablecoins from a monetary perspective. Salehi et al. \cite{dai_liquidation} explore the liquidation process in stablecoins, and put forward a research agenda for alternatives to liquidation. Clements R. \cite{clements2021builttofail} studies the inherent fragility in algorithmic stablecoins and claims that they are built to fail. Zhao et al. \cite{volatility} conduct an empirical analysis to explain the volatility of algorithmic stablecoins.

==> Section/others.tex <==
% An arbitrageur can extract risk-free profit when 1 TerraSDR $=0.9$ SDR by trading TerraSDR for 1 SDR's worth of Luna from the system, as opposed to $0.9$ SDR's worth of assets she could get from the open market.
% Similarly, she can also extract risk-free profit when 1 TerraSDR $=1.1$ SDR by trading in 1 SDR worth of Luna to the system to get $1.1 \mathrm{SDR}$ worth of TerraSDR, once again beating the price of the open market.

% To maintain its stablecoins' equilibrium, Terra mints and burns tokens while also incentivizing arbitrage.
% Before one can buy UST, you'll have to mint some.
% To do so, you'll pay the going rate in LUNA. The protocol takes those LUNA and burns them, which constricts their supply and makes the price of LUNA go up just a bit. The same works in reverse: to mint LUNA, you'll convert UST stablecoins. Those get burned and the price of UST goes up ever so slightly.

% % Why might you want to do this?
% In addition to using the assets for some service or utility, there's a potential arbitrage opportunity. Arbitrageurs—traders who profit from small price discrepancies—help to keep the price of UST in check by selling LUNA for UST when the price of UST is below \$1 and buying LUNA when UST is worth more than \$1. If, for example, UST slips to \$0.95, traders can then buy a bunch at that price but sell it for \$1 of LUNA. In doing so, UST supply is reduced and, therefore, the price heads back up—at least, in theory.

% So, under what circumstances will lenders agree to be part of a rational Ponzi game?
% The basic result that has been established is that Ponzi games require the participation of an infinity of agents~\cite{ponzi_rational}.
% With an infinite number of agents over time, by contrast, there always exists a new set of agents with whom to trade, and this may make it possible for debt to be rolled over perpetually.
% The introduction of perpetually rolled over debt will never make the lending economy worse off and will in general make it better off relative to a world in which no Ponzi game is run.

As total demand for the stablecoin increases or decreases, the supply automatically changes in response. While different projects use different methods to expand and contract the stablecoin supply, the most commonly used is the “bonds and shares” method introduced by Basis cash.

As the network grows, so too does demand for the stablecoins. Given fixed supply, an increase in demand will cause the price to increase. In the seigniorage shares model, however, increased demand causes the system to issue new stablecoins, thus increasing supply, and ultimately lowering price to the target level. This works conversely, using “bonds” to remove coins from circulation (more details below).

The major challenge of seigniorage shares is figuring out how to increase and decrease the monetary supply in a way that is both decentralized, resilient, and ungameable. Expanding the money supply is easy: print money! Contracting the money supply, on the other hand, is not. Who loses money? Is it forced, or voluntary? If voluntary, what motivation does the person have to part ways with her stablecoin?

Stablecoins that rely on debt marketplaces, i.e., bonds, to regulate supply, will always rely on lenders of last resort, i.e., bailouts.
We have seen this in traditional markets, we say this with makerDAO.
It is true of basis cash, terraUSD as well.

Cryptocurrencies like Bitcoin govern the supply of coin through simple and deterministic coin growth rules.
As a result, unanticipated changes in coin demand are reflected in changes in coin price, causing volatility and discouraging usage of coin as media-of-exchange.
Seigniorage shares~\cite{noteonshares}
argue that next-generation cryptocurrencies should incorporate an elastic supply rule that adjust the quantity of coin supply proportionately to changes in coin market value.

In a coin stabilisation scheme, changes in coin price stand proxy for changes in coin demand, and coin supply changes in response to changes in coin price. The idea is that an $X \%$ change in coin price, followed by an $X \%$ change in coin supply, will return coin price to its initial value, as as represented by the green box.

So the core operational principle of a protocol that aims to stabilise the market value of coin is the following rule: at the end of some pre-defined interval of time, if the change in coin price over the interval is $X \%$, change coin supply by $X \%$. More specifically, let's call that interval of time the rebase period, defined as every $n$ blocks. The coin supply rule mandates that:
$$
\begin{aligned}
Q_{i} &=Q_{i-1} \times \frac{P_{i}}{P_{i-1}} \\
\Delta_{i} &=Q_{i}-Q_{i-1}
\end{aligned}
$$
, where $i$ is the $\mathrm{i}-\mathrm{th}$ rebase period, $Q$ is coin supply and $P$ is coin price.

The solution to coin distribution offered, Seigniorage Shares, suggestS that there needs to be two types of coin: coin that acts like money and coin that acts like shares in the system's seigniorage.
For short, we'll just call these coins and shares. Coins and shares are identical in all respects (transaction verification works via ECDSA signature, etc) except for the process that regulates their respective supply.

Coins are the object of stabilisation, and $\Delta_{i}$ of coin is distributed to the holders of shares. When coin supply needs to increase, coinbase is distributed to share holders in exchange for a certain percentage of shares, which are destroyed (coin supply increases, share supply decreases). When coin supply needs to decrease, sharebase is distributed to coin holders in exchange for a certain percentage of coin, which are destroyed (coin supply decreases, share supply increases).

The mechanism of these shares-for-coin and coinfor-shares swaps is a voluntary one, a decentralised auction the rules of which are written into the protocol. The quantity of coins to create or destroy is defined via the $\Delta_{i}$ process in equations 3 and 4 , and there is an auction at the end of every rebase period.
When $\Delta_{i}$ is positive (new coins need to be created) a coin auction for $\Delta_{i}$ coins begins at the block or ledger set defining the start of rebase period $i+1$. Any holder of shares can bid for coins by signing and broadcasting a special TX describing the quantity of shares he is willing to trade for coin, and the minimum coins/shares price that he will accept. Winning bids are filled at whatever coins/shares price $P^{s}$ that clears the quantity to be sold. So $\Delta_{i}$ new coins are distributed to the winning bidders and $\Delta_{i} / P^{s}$ shares are destroyed. ${ }^{2}$

When $\Delta_{i}$ is negative (some existing coins need to be destroyed), a share auction of $\Delta_{i}$ worth of shares begins. Holders of coin can submit bids to purchase shares, signing a special TX describing the quantity of coins he is will to trade for shares, and the maximum coins/shares price $P^{s}$ that he will accept. Winning bids are filled at whatever price clears the quantity to be sold. So $\Delta_{i} / P^{s}$ new shares are distributed to the winning bidders and $\Delta_{i}$ coins are destroyed.

If the long-run demand for coin is positive, coin supply will increase with demand, but the quantity of shares will get increasingly scarce.






%1 讲一讲我理解的 $OHM 。首先说我非常看好项目。争议很多是因为超高APY看起来很像旁氏。但事实是这个“旁氏”越来越接近成功，尤其是经过519以及昨天的过山车考验之后。

%2 协议定位跟之前的算稳项目都不同，没有要求锚定1美元。这是一个非常聪明的决定，协议策略是首先吸纳足够多的资金(ProtocolControlledValue)，先壮大实力再去考虑其他目标。协议是backed, not pegged。

%3 $OHM 最成功的是引入了博弈论，对参与者来说越早参与获利越多，对于整个群体来说，所有都stake 是获利最大的解，这也是项目meme 3，3 的由来

%4 $OHM 的创新是通过出售bond的方式吸引更多资金锁定到PCV，用户通过bond获得折扣，协议通过bond锁定更多资金，属于双赢。这也反映了创始人 @ohmzeus的哲学： 拥有/购买流动性优于租赁流动性。
Ponzi, a design that old liability should be financed by issuing new debt,
Ponzi, a design that old liability should be financed by issuing new debt, has always been instinctively resented by the public.
Ponzi schemes,
where individuals or companies pay out funds to some parties by borrowing funds from others,


% Ponzi schemes normally share some common characteristics, and U.S. Securities and Exchange Commission~\cite{ponzi_gov} raises ``red flags'' for these warning signs, namely
% (1) high returns with little or no risk;
% (2) overly consistent returns;
% (3) unregistered investments;
% (4) unlicensed sellers;
% (5) secretive, complex strategies;
% (6) issues with paperwork;
% (7) difficulty receiving payments.
% Ponzi schemes are named after Charles Ponzi, who duped investors in the 1920s with a postage stamp speculation scheme.
% Ponzi scheme organizers often promise to invest your money and generate high returns with little or no risk.
% But in many Ponzi schemes, the fraudsters do not invest the money.
% Instead, they use it to pay those who invested earlier and may keep some for themselves.
% a Ponzi can be an investment fraud that pays existing investors with funds collected from new ones.
% where individuals or companies pay out funds to some parties by borrowing funds from others.

Fiat-collateralized stablecoins are pegged to the value of fiat, most often USD.
Fiat collateral remains in reserve with the central issuer and must reflect the number of corresponding stablecoins in circulation.
Collateralized: the stablecoin is a digital representation of the funds that collateralise it and every unit represents a claim on the issuer over the funds it receives from the users.
Crypto-collateralized: digital assets provide the backing rather that banks or cash using CDPs or collateralized debt positions.
Dai the first unbiased currency, over-collateralized
Frax, fractional-algorithmic stablecoin, being partially backed by collateral and partially stabilized algorithmically

Basis Cash~\cite{basiscash} is an Algorithmic Stablecoin
Pegged to 1 USD.
The protocol is designed to expand and contract supply similar to the way central banks trade fiscal debt to stabilize purchasing power, without any rebases or collateral risk.

Although there exists a wide variety of stablecoin mechanisms, Basis Cash specifically uses an “algorithmic central bank” approach to manage the supply of tokens according to a predetermined logic. The algorithm is in charge of balancing stablecoin supply to fluctuating demand, ensuring that the token price remains relatively stable.

There are three tokens in the Basis Cash design.
BAC - Basis Cash.
Basis Cash tokens are designed to be used as a medium of exchange. The built-in stability mechanism expands and contracts their supply, maintaining their peg to the MakerDAO Multi-Collateral Dai token (which roughly trades near the United States Dollar).

BAB - Basis Bonds.
Basis Bonds are minted and redeemed to incentivize changes in the Basis Cash supply. Bonds are always on sale to Basis Cash holders, although purchases are expected to be made at a price below 1 Basis Cash. At any given time, holders are able to exchange their bonds to Basis Cash tokens in the Basis Cash Treasury. Upon redemption, they are able to convert 1 Basis Bond to 1 Basis Cash, earning them a premium on their previous bond purchases.
Contrary to Basis Bonds of basis.io, bonds in Basis Cash do not have expiration dates. All holders are able to convert their bonds to Basis Cash tokens, as long as the Treasury has a positive BAC balance.

BAS - Basis Shares.
Basis Shares loosely represent the value of the Basis Cash network. Increased demand for Basis Cash results in new Basis Cash tokens to be minted and distributed to Basis Share holders, provided that the Treasury is sufficiently full.
Holders of Basis Share tokens can claim a pro-rata share of Basis Cash tokens accumulated to the Boardroom contract.

Tokens Distributed through
Yield Farming.
BAC and BAS tokens are distributed fairly through yield farming. Providing liquidity to BAC-DAI and BAS-DAI pairs result in additional BAS tokens being distributed.
This not only allows us to maintain our censorship resistance, but also acts as an incentive mechanism against lack of liquidity and bond death spirals — as famously pointed out with the original Basis.

When the price is above \$1
Basis Cash supply is expanded to bring the price back down. The ones who staked Basis Shares on the Boardroom will receive BAC seigniorage as rewards.
When the price is below \$1
The protocol auctions off Basis Bonds for BAC to contract Basis Cash supply. They can be redeemed for premiums after BAC price returns to its 1 dollar peg.

==> [CryptEx23] Rational Ponzi Game in Algorithmic Stablecoin/Section/1intro.tex <==
\section{Introduction}
\label{sec:intro}
Ponzi is making a comeback that is used to describe the hyped algorithmic stablecoins today. The most recent critique was directed at the one called TerraUSD (UST), which crashed by almost 98\% within 24 hours on May 12$^{\text{th}}$, 2022 (cf.\cite{coinmarketcap}), impacting a direct of \$85B market value evaporation and the collapse of entire crypto markets. This worst-hit reveals a new type of bank run and has triggered repetitive rounds of criticism and discussion about the stablecoin and its algorithmic stabilized approaches. Stablecoins are created to share all great features that cryptocurrencies hold (e.g., decentralization, automation, cross-border), without, however, suffering from the same volatility, making them much more applicable as a store of value, medium of exchange, and unit of account~\cite{sokemin,stablecoins2.0,demys_stable}.
In an ideal form, stablecoins are simply cryptocurrencies with stable value. Current stablecoin implementations (cf. Tab.\ref{tab:stablecoin}) aim to bridge external assets with the cryptocurrency space by anchoring a peg (e.g., USD) in price. 

\input{table/stablecoins}


Stablecoins in cryptocurrencies are generally tagged as either collateralized or algorithmic stablecoins in terms of their specific collaterals. The collateralized stablecoin, as the name implies, requires collateral and thus ensures the circulating token having a redemption value. Possible collateral options include fiat money, cryptocurrency, and other valuable assets.
Currently, stablecoins are majorly backed by fiat money (Tab.\ref{tab:stablecoin}). USDC \cite{usdc}, for example, is a fully collateralized stablecoin pegged to USD and stores its US dollars in a number of banks. Such a type of stablecoins, backed by fiat money, are generally of a high degree of centralization. Instead, using cryptocurrencies as collateral can circumvent this problem. However, considering the high volatility, an \textit{over}-collateralization is thereby required if relying on cryptocurrencies as collateral.  One representative in this category is the stablecoin DAI \cite{dai}, where a user needs to deposit Ether (the native token of Ethereum) in excess of the amount of created DAIs. Even if the collateral crypto depreciates, each unit of the stablecoin still has enough space of being redeemed for at least an equivalent amount of underlying assets.


Algorithmic stablecoin (AS), however, does \textit{not} require any collateral. The money supply of algorithmic stablecoin is elastic and managed by algorithms (i.e., coded in smart contracts). Algorithmic stablecoins are thus not limited in scale by the circulating amount of the underlying collateral. For stabilization, the par value of an algorithmic stablecoin is basically preserved by expanding supply when the price is too high and contracting it when the price is too low. Two distinct AS designs are prevailing in markets \cite{volatility}, namely, \textit{rebase} and \textit{seigniorage shares}. 
Rebase~\cite{hayekrebase} is an algorithm that automatically adjusts the money supply in response to the market demand on a routine basis. A rebase protocol can add (\texttt{mint}) or remove (\texttt{burn}) coins from circulation according to the stablecoin's price deviation from the peg, and this is normally achieved by adjusting token balance pro rata across all wallets. Instead of rebasing one coin, seigniorage shares~\cite{noteonshares} normally has a \textit{dual} (or \textit{multiple}) coin design: the price-stable coins and flexible investment shares. The shares algorithmically expand and contract the supply of price-stable coins much like a central bank does with fiat currencies. Seigniorage shares model has, to varying degrees, served as a foundation for TerraUSD \cite{TerraUSD}, Empty Set \cite{emptyset}, Basis Cash \cite{basiscash}, and Frax \cite{frax}.

\smallskip
\noindent\textbf{Contributions.} Unfortunately, no satisfactory algorithmic stablecoins have been healthily operated for a long-term run. Non-stable performance and non-collateral property destroy the natural trust of participants and communities. AS schemes are thus often questioned as Ponzi schemes. This motivates our observations towards this fancy but fuzzy concept. \textit{\text{First}}, we comprehensively review existing in-the-wild AS projects and 
explore the design primitives they share in common (Sec.\ref{sec:intro}). \textit{\text{Then}}, we accordingly have established a rational Ponzi model in the context of algorithmic stablecoins (Sec.\ref{sec:model}) and \textit{\text{further}} evaluate two mainstream projects, namely, Ampleforth and TerraUSD (the representatives of \text{Rebase} and \text{Seigniorage share}, respectively), based on six-month historical data from Mar 1$^\text{st}$ to Oct 17$^\text{th}$ 2022 (Sec.\ref{sec:apply}). \textit{\text{Also}}, we find several interesting insights (Sec.\ref{sec:discuss}) that are driven by our model. \textit{\text{Last}}, we deliver a taking-home message saying: \textit{the rebase approach is much more likely to achieve a rational Ponzi game as long as it always exists in an active trading market whereas the seigniorage share method is, if without external interruptions, of low probability to realize it due to the uncontrollable death spirals from the overlapped effect of dual coins}.




\smallskip
\noindent\textbf{Recent Studies.} 
A series of papers and reports~\cite{demys_stable,designstablecoins,stablecoinsurvey,multicoinsry} establish and extend the taxonomies in stablecoins based on the peg type, the collateral type, and the collateral amount. They give an initial sight to demystify its assemblies and components. Besides, with in-depth analysis, a bunch of follow-up works is proposed.  Moin et al. \cite{sokemin} provide a systematical classification of existing stablecoins in terms of their design elements.  Ariah et al. \cite{stablecoins2.0} explore the economic structure of stablecoins and establish a risk-based functional characterization. Pernice et al. \cite{openquestion} research stablecoins from a monetary perspective. Salehi et al. \cite{dai_liquidation} explore the liquidation process in stablecoins, and put forward a research agenda for alternatives to liquidation. Clements R. \cite{clements2021builttofail} studies the inherent fragility in algorithmic stablecoins and claims that they are built to fail. Zhao et al. \cite{volatility} conduct an empirical analysis to explain the volatility of algorithmic stablecoins.



% A paper by Pernice et. al takes a different approach, categorizing stablecoins by monetary and exchange rate regimes [53].

% Studies investigating the asset class and its manifestations include [cite] and [cite].
% The user perception in the adoption of stablecoins has been studied in [], while [] analyzed the suitability of stablecoins as save-haven investment.
% The relation between cryptocurrency prices and stablecoin trading has been focused on by [] and []. 
% Adopting a risk-oriented approach, [] and [] suggest theoretic models to study stability and resilience of stablecoins. While the latter focuses on extreme events, [] not only offers a theoretic model for day-to-day arbitrage but also provides, to my knowledge, the first extensive empirical analysis of the drivers of stablecoin prices. 



% \begin{wraptable}{r}{5cm}
%  \caption{Stablecoin Category} 
%  \label{tab:stablecoin}
%   \centering
%  \resizebox{\linewidth}{!}{ \begin{tabular}{l r}
%     \toprule
%       & \textbf{Collateral Type}  \\
%     \midrule
%     \multirow{3}{*}{\textit{Collateral}}  &  Fiat collateral  \\
%       &  Crypto collateral  \\
%       &  Other collateral  \\
%     \cmidrule{1-2}
%     \textit{Partial-collateral}  & - \\ 
%     \cmidrule{1-2}
%     \multirow{2}{*}{\textit{\makecell{Algorithmic \\(non-collateral)}}} & \cellcolor{pink} Rebase \\
%     &  \cellcolor{pink} Seigniorage shares \\
%     \bottomrule
%   \end{tabular}}
%   \label{server}
% \end{wraptable}
% % blue!25



% https://drive.google.com/file/d/1BADClaZBZhXkYdsMxaJ6icJhNFlWuvV9/view?usp=sharing


% However, the cryptocurrency collateral itself is highly volatile,
% compared to fiat currency,
% thus making it hard to use as a guarantee of value.
% Crypto collateral are managed by smart contract, a self-executing program, thus eliminating the dependence on a third party.
% Specifically, collateral deposit can be accessed by paying back the stablecoin debt, or can be automatically liquidated if the value of collateral falls below a certain threshold.






% \noindent\textbf{Roadmap.} 
% The roadmap of this work is as follows.
% We briefly review related works in Section~\ref{sec:relatedwork}.
% % In Section~\ref{sec:background}, we break down the taxonomy of stablecoins as collateral stablecoin and algorithmic stablecoin (i.e., without collateral, abbreviated as AS).
% % In Section~\ref{sec:background}, we investigate the classification of algorithmic stablecoin (i.e., without collateral, abbreviated as AS) and their corresponding mechanics.
% In Section~\ref{sec:model}, we construct a concise model of rational Ponzi game.
% We then examine whether Ampleforth (rebase) and TerraUSD (Seigniorage Shares) meet the conditions of being rational Ponzi games.
% Finally, we provide conclusion remarks in Section~\ref{sec:conclusion}.




==> [CryptEx23] Rational Ponzi Game in Algorithmic Stablecoin/Section/2model.tex <==
\section{Modeling Rational Ponzi Games}
\label{sec:model}

Ponzi~\cite{ponzi_wiki} has always been such a term that is instinctively resented by the public. For malicious organizers, Ponzi schemes are used to lure new investors, and leverage incoming money to pay earlier ones while keeping the rest as profit.
In general, organizers will promise an abnormally high return to investors within the short term. With little or no legitimate earnings, Ponzi games require a constant flow of new funds to survive. Once becoming difficult to recruit new participants, or whenever a large number of existing investors cash out, these games tend to collapse. 
However, stemming from its origin, the substance of Ponzi is neutral yet subtle. Economists~\cite{ponzi_minsky,ponzi_kindleberger} discuss a perfect foresight version of the Ponzi model, where the schemes based on imperfect information or irrationality of lenders are ruled out. They call such a policy, in which all repayments are forever \textit{rolled over}, i.e., financed by issuing new debt, a \textit{rational Ponzi game}~\cite{ponzi_rational}. Following such narrative connotations, we develop the model in the context of algorithmic stablecoins. 


% By engaging in a Ponzi game, the borrower is able to extract positive resources (in present value terms) from the lender(s). The classic form of this scheme consists of borrowing money (issuing short or long term debt) and financing all promised payments of principal or interest by issuing new debt. 

% sequence

\smallskip
\noindent\textbf{Rational Ponzi Game.}
An entity that plans to issue debt and roll it over the possibly infinite future is the borrowing side of a rational Ponzi game. Any plan will impose a set of net cash inflows $I_s$ from the lending side. The present value of borrower's net indebtedness $D_{T}$ of at any time $T$ equals the present value of the stream of prospective incomes generated by lenders between $0$ and $T$:

\begin{equation}
\Gamma(T) D_{T}=\sum_{s=1}^{T} \Gamma(s) I_{s}
\end{equation}
where $\Gamma(T)$ is the discount factor of the borrowing side, it is calculated by the interest rate $r_{t}$ between periods $t-1$ and $t$\footnote{In corporate finance, a discount factor is a number that is derived from the discount rate. It is used to discount future cash flows back to their present value at a specific discount rate. Here, we assume $r_{t}$ are identical for all assets under perfect foresight.}, and $\Gamma(s)$ is the discount factor applicable in period 0 to cash inflows received in the period $s$, where
$ \Gamma(s) \equiv \prod_{j=1}^{s}\left(1+r_{j}\right)^{-1}.$ 
We now provide the definition of a rational Ponzi game.

\begin{defi}[Rational Ponzi Game]\label{defi-ponzi}
A rational Ponzi game is a sequence of debt transactions satisfying the following sense: \begin{itemize}
    \item[(i)] to the borrower, it is a positive net present indebtedness value such that $\lim _{T \rightarrow \infty}$ $\Gamma(T) D_T>0$, if the limit of $\Gamma(T) D_T$ exists;
    \item[(ii)] to all the participants, i.e., both the borrowing and lending sides, the game enables a Pareto improvement\footnote{A Pareto improvement is an improvement to a given situation, where a change in allocation of goods harms no one and benefits at least one individual.}.
\end{itemize}
\end{defi}

The first holding condition in Definition 1 implies that debts 
are unnecessarily fully paid off by future cash inflows if in an infinite horizon setting. The second condition imposes restrictions that no one is being worse (assets can always be redeemed at least equal to the market value of assets deposited). Therefore, the two conditions guarantee a rational realization. We provide a general operation process of rational Ponzi schemes as in Fig~\ref{fig:rational}. The red plus sign and the green minus sign represent cash inflow and cash outflow, respectively. The values in parentheses following each participant represent their corresponding utility.


%you can edit the figure here: https://drive.google.com/file/d/1yK-DRCSBQIFNEzGlQW87cfWnQ03dqLj7/view?usp=sharing

\begin{figure}[H]
	\centering
	\includegraphics[scale=0.56]{figs/rational_ponzi_demo.pdf}
	\vspace{-0.3cm}
	\caption{A general flow interpreting how a rational Ponzi game works.} 
	\label{fig:rational}
 	\vspace{-0.5cm} 
\end{figure}

\noindent\textbf{Scope of application.} One may consider that only governments are entitled to run such rational Ponzi games. However, in a world where rational Ponzi games can exist, any infinitely lived entity can issue debt and perpetually roll it over. In principle, even a finitely lived entity can issue bonds with zero coupon, i.e., fiat money. All required is to make participants believe that there will always exist followers being willing to purchase the debt. Meanwhile, economists have proven that the introduction of perpetually rolled over debt will never make the lending economy worse off relative to a world in which no Ponzi game runs~\cite{ponzi_rational,tirole1985asset,pernice2019monetary}.




\section{Applied to Algorithmic Stablecoins}
\label{sec:apply}

Typically, algorithmic stablecoins, based on their operating mechanisms, can be considered a Ponzi game: an on-chain protocol launches a coin (equiv. debt) claimed to be stable (investors can always obtain the equivalent fund back when selling the coin), and one joins the game by purchasing the coin and can quit the game if others are willing to buy his coins on the market. However, is such an algorithmic stablecoin game \textit{rational} under our model? In this section, we instigate two typical instances, Ampleforth (rebase) and TerraUSD (seigniorage shares), to answer this question.
Supposing that all the lending protocols are deployed on smart contracts on a public ledger so that all steps are perfectly enforceable (equiv. no default risk). We define the notation $\mathcal{U}$ as the investor's utility; it is basically the product of the number of held assets $Q$ and the market price of the token $P$, in symbols as
\begin{equation}
\mathcal{U} = Q \times P.
\end{equation}

Then, we apply our model to two concrete instances by investigating their six-month historical data (Mar\,--\,Oct, 2022). We analyze the utility of investors based on extracted data covering price, quantity, and market cap.

\smallskip
\noindent\textbf{Ampleforth.} 
Ampleforth (AMPL) \cite{ampleforth} is an algorithmic stablecoin protocol that applies the design of rebase. AMPL is pegged to the CPI-adjusted USD, and its rebase procedure occurs at 02:00 UTC on a daily basis. The quantity of AMPL tokens in user accounts automatically expands or contracts based on everyday price.
% The rebase() method first queries the Market Oracle to get the current price. If the price is within priceThreshold of the target price, no supply policy change is applied.
%
According to Ampleforth white paper~\cite{amplwhiterpaper}, the absolute \texttt{supplyDelta} of AMPL is equal to \texttt{(price-target)*totalSupply/target}.
For example, at the time of rebase, if the price of AMPL is \$1.1, 10\% greater than the standard 1 USD peg, a wallet with a balance of 100 AMPL will be rebased as 110 accordingly. In contrast, when the AMPL price is less than 1 USD, the protocol will proportionally decrease the quantity of tokens in wallets, aiming to bring the price up to its anchor.


\begin{figure}[!hbt]
	\centering
	\includegraphics[width=1\textwidth]{figs/ampf.png}
	\caption{AMPL price, number of AMPL, and investor's utility over time.}
	\label{fig:ampl}
\vspace{-0.4cm}
\end{figure}


\smallskip
\noindent\textit{Investor's utility analysis.}
Considering an investor who participates in the Ampleforth game at any time by purchasing one unit of AMPL, we analyze the changes in his utility over time. At each rebase time (cf. Fig.\ref{fig:ampl}), the investor's utility (red line) stays the same\footnote{Except for the rebase time in a day, the number of AMPL in wallets will not change. If the coin price rises and the investor selects to sell, his utility is greater than his original investment.}, meaning that the investor can always redeem (trade) the identical value of his investment back. However, the price of AMPL (green line) cannot keep stable, and the AMPL balance (blue line)\footnote{To better demonstrate the nature of rebase, we calculate daily AMPL numbers based on a simple settings from its 1st version whitepaper~\cite{amplwhiterpaper}.} is in the investor's wallet. In terms of a rational Ponzi model, AMPL has the potential to satisfy all listed conditions as long as there exists an lively traded market. 

Since any investor can retain at least the same utility in the AMPL network, regardless of the price of the token, one may wonder why the rebase is not being adopted on a larger scale. The most obvious reason is due to its highly volatile price, resulting in holding AMPL being no different than holding a regular cryptocurrency. At the same time, one's balance varies proportionally to the price every day, making the holder fall into passive and anxious emotions. Besides, AMPL, as an ERC-20 token that works natively on Ethereum blockchain, cannot perform its rebase implementation smoothly in a centralized exchange or other blockchain platforms, significantly restricting its use scenarios. Ampleforth mitigates this constraint with the release of Wrapped-AMPL, a token that wraps AMPL similar to wrapped ETH. Wrapped-AMPL facilitates ecosystem integrations on both centralized and decentralized platforms. 


\smallskip
\noindent\textbf{TerraUSD.} 
TerraUSD (UST) \cite{TerraUSD} is a seiniorage shares style stablecoin pegging to the USD on top of Terra's blockchain. LUNA, as the native staking token of the Terra blockchain, absorbs the volatility from UST.
Aibitrage can help making UST price stable: when the UST's price is $<1$ USD, arbitragers can send 1 UST to the system and receive 1 USD's worth of LUNA; whereas the UST's price becomes $>1$ USD, arbitragers will send 1 USD's worth of LUNA to the system and receive 1 UST.

\begin{figure}[!hbt]
	\centering
	\includegraphics[width=1\textwidth]{figs/ust.png}
	\caption{UST price, number of UST, and investor's utility over time.} 
	\label{fig:ust}
	\vspace{-0.3cm}
\end{figure}


\noindent\textit{Investor's utility analysis.}
We also consider an investor who participates in the UST game at any time by purchasing one unit of UST. For simplicity, we assume that the investor will always hold UST without converting him to LUNA in the mid-run before exiting the game.  A chart of UST price (green line), the number of UST in the wallet (red line), and the investor's utility (blue line) over time are presented in Fig.\ref{fig:ust}.
The practice proves the ineffectiveness of UST's stabilization as the UST eventually collapsed.
Investors suffered a significant loss from their initial investments,
% even though the token claimed its value could stay stable.
making UST unlikely to become a rational Ponzi game.
% We here examine the reasons that result in such failure by finding the unsatisfied requirements defined in our rational model.

In fact, current designs of seigniorage shares are practically difficult for realizing a rational model. These stablecoins are not substantially secured by anything, other than the expectation that the stablecoin will eventually appreciate in value. Hence, a necessary condition for the seigniorage shares to work healthy is that the secondary coin has to have values. LUNA, as the secondary coin, should have, at least, trading values, as people do use Terra blockchain every day. However, in extreme cases, investors may still lose confidence in it, and the massive sell-off has accelerated both two types of coins into a death spiral faster.


% non-pegged coin: 
% death spriral is the key why not achieve rational to such design.
% If there is a malicious actor intent on sabotaging the stability,
% 3 cases: price up, flat, down.

% As long as people are using the Terra/Luna blockchain, Terra should retain some value.
% Fees and rewards, also paid in Luna, are additionally adjusted to entice users to buy and hold Luna even during downturns.




==> [CryptEx23] Rational Ponzi Game in Algorithmic Stablecoin/Section/3discuss.tex <==
\section{Discussion}
\label{sec:discuss}

\noindent\textbf{Market cap vs price stability.}
The investors involved in stablecoin markets often have intuitive feelings that the larger the market cap of the stablecoin, the better stability the stablecoin can achieve with regard to its peg. However, according to the price and market cap data from CoinGecko \cite{coingecko}, this conjecture may not be valid as imagined for algorithmic stablecoins. The statement of ineffective application to the rebase design is explicit, as its market capitalization will vary as the supply of the currency is adjusted. For the seigniorage share design, this statement will be invalid as well. Due to its relative complexity, there are a lot of possibilities resulting in this situation, one of which is the loss of confidence. The recent joint collapse of LUNA/UST was a loop in which the market lost confidence and entered a death spiral, pushing them out of the market cap top 10 within merely several hours. Thus, a larger market cap in algorithmic stablecoin does not necessarily guarantee better stability.


\smallskip
\noindent\textbf{Price oracle risk.}
Price oracle provides the price feed for on-chain DeFi protocols \cite{werner2021sok}, and it is crucial to the secure operation of an algorithmic stablecoin. Algorithmic stablecoins may have special price-feeding needs due to the existence of algorithms, which further need to establish their own oracles. An internal oracle, however, will inevitably lead to an additional layer with potential centralization and incentivize the coin issuer to update the price in his favor. In contrast, opting for an external price oracle may mitigate this problem, but it is still vulnerable to external price manipulation, being out of the control of the coin issuer. Relevant attacks include flash loan price manipulation attack, pump, and dump~\cite{Attackflashloan}. Selecting a trustworthy price oracle is not easy for an algorithmic stablecoin, and a comprehensive ex-ante risk assessment is required.

\smallskip
\noindent\textbf{Reconsider the necessity of a peg.}
Stablecoins are designed to be pegged to some underlying assets, with the USD being a popular choice. Anchoring a benchmark is an effective way to achieve stability in stablecoins. People may thus generally assume a fact that the stablecoin is perfectly fungible for its peg. However, this is not the full truth. Stablecoins can be, in fact, rather considered as their own free-floating assets that closely track the value of a peg. Besides, it is also possible that stablecoins could provide the desired stability without pegging to an asset. In one possible future, once the economy develops surrounding the stablecoin itself, and such stablecoins have also been widely used as a medium of exchange, maintaining a perfect peg becomes unnecessary.




% \begin{figure}[!hbt]
% 	\centering
% 	\includegraphics[width=1\textwidth]{figs/marketcap.png}
% 	\caption{Market Cap and Utility.} 
% 	\label{fig:marketcap}
% \end{figure}


==> [CryptEx23] Rational Ponzi Game in Algorithmic Stablecoin/Section/4conclude.tex <==
\section{Concluding Remarks}\label{sec:conclu}
% This study creatively applies O'Connell \& Zeldes's model (1988, cf.\cite{ponzi_rational}) to the context of algorithmic stablecoins.
% Following its connotation, we establish a rational Ponzi game as the measurement and accordingly evaluate two mainstream algorithmic stablecoin projects (Ampleforth and TerraUSD) as instances.

This study creatively applies O'Connell \& Zeldes's model (1988, cf.\cite{ponzi_rational}) for rational Ponzi games to the context of algorithmic stablecoins. Our analyses of investors' utilities indicate that the rebase approach has the potential to realize a rational Ponzi game as long as it always exists in an active trading market. Notably, by leveraging smart contracts, DeFi protocols will be much easier to realize a rational Ponzi model than those in centralized finance, by means of many advanced and innovative financial tools like automated market makers (AMM), flash loans, and enforceable payment. In contrast, the seigniorage share method is difficult to guarantee a rational Ponzi, as dealing with the selling pressure in a death spiral for dual coins is intrinsically complicated. Beyond that, we point out the hurdles existing in current algorithmic stablecoin implementations and further identify the potential opportunities for future endeavors. 
% To the best of our knowledge, this paper proposes the first study for identifying, establishing, deciding, and evaluating rational Ponzi games in the track of algorithmic stablecoins. 


% and put forward a research agenda for alternatives to ration model in algorithmic stabecoins.



==> [CryptEx23] Rational Ponzi Game in Algorithmic Stablecoin/Section/5releatedwork.tex <==
\section{Related Works}
\label{sec:related}
% \noindent\textbf{Recent Studies.} 
A series of papers and reports~\cite{demys_stable,designstablecoins,stablecoinsurvey,multicoinsry} establish and extend the taxonomies in stablecoins based on the peg type, the collateral type, and the collateral amount. They give an initial sight to demystify its assemblies and components. Besides, with in-depth analysis, a bunch of follow-up works is proposed.  Moin et al. \cite{sokemin} provide a systematical classification of existing stablecoins in terms of their design elements.  Ariah et al. \cite{stablecoins2.0} explore the economic structure of stablecoins and establish a risk-based functional characterization. Pernice et al. \cite{openquestion} research stablecoins from a monetary perspective. Salehi et al. \cite{dai_liquidation} explore the liquidation process in stablecoins, and put forward a research agenda for alternatives to liquidation. Clements R. \cite{clements2021builttofail} studies the inherent fragility in algorithmic stablecoins and claims that they are built to fail. Zhao et al. \cite{volatility} conduct an empirical analysis to explain the volatility of algorithmic stablecoins.

==> [CryptEx23] Rational Ponzi Game in Algorithmic Stablecoin/Section/others.tex <==
% An arbitrageur can extract risk-free profit when 1 TerraSDR $=0.9$ SDR by trading TerraSDR for 1 SDR's worth of Luna from the system, as opposed to $0.9$ SDR's worth of assets she could get from the open market.
% Similarly, she can also extract risk-free profit when 1 TerraSDR $=1.1$ SDR by trading in 1 SDR worth of Luna to the system to get $1.1 \mathrm{SDR}$ worth of TerraSDR, once again beating the price of the open market.

% To maintain its stablecoins' equilibrium, Terra mints and burns tokens while also incentivizing arbitrage.
% Before one can buy UST, you'll have to mint some.
% To do so, you'll pay the going rate in LUNA. The protocol takes those LUNA and burns them, which constricts their supply and makes the price of LUNA go up just a bit. The same works in reverse: to mint LUNA, you'll convert UST stablecoins. Those get burned and the price of UST goes up ever so slightly.

% % Why might you want to do this?
% In addition to using the assets for some service or utility, there's a potential arbitrage opportunity. Arbitrageurs—traders who profit from small price discrepancies—help to keep the price of UST in check by selling LUNA for UST when the price of UST is below \$1 and buying LUNA when UST is worth more than \$1. If, for example, UST slips to \$0.95, traders can then buy a bunch at that price but sell it for \$1 of LUNA. In doing so, UST supply is reduced and, therefore, the price heads back up—at least, in theory.

% So, under what circumstances will lenders agree to be part of a rational Ponzi game?
% The basic result that has been established is that Ponzi games require the participation of an infinity of agents~\cite{ponzi_rational}.
% With an infinite number of agents over time, by contrast, there always exists a new set of agents with whom to trade, and this may make it possible for debt to be rolled over perpetually.
% The introduction of perpetually rolled over debt will never make the lending economy worse off and will in general make it better off relative to a world in which no Ponzi game is run.

As total demand for the stablecoin increases or decreases, the supply automatically changes in response. While different projects use different methods to expand and contract the stablecoin supply, the most commonly used is the “bonds and shares” method introduced by Basis cash.

As the network grows, so too does demand for the stablecoins. Given fixed supply, an increase in demand will cause the price to increase. In the seigniorage shares model, however, increased demand causes the system to issue new stablecoins, thus increasing supply, and ultimately lowering price to the target level. This works conversely, using “bonds” to remove coins from circulation (more details below).

The major challenge of seigniorage shares is figuring out how to increase and decrease the monetary supply in a way that is both decentralized, resilient, and ungameable. Expanding the money supply is easy: print money! Contracting the money supply, on the other hand, is not. Who loses money? Is it forced, or voluntary? If voluntary, what motivation does the person have to part ways with her stablecoin?

Stablecoins that rely on debt marketplaces, i.e., bonds, to regulate supply, will always rely on lenders of last resort, i.e., bailouts.
We have seen this in traditional markets, we say this with makerDAO.
It is true of basis cash, terraUSD as well.

Cryptocurrencies like Bitcoin govern the supply of coin through simple and deterministic coin growth rules.
As a result, unanticipated changes in coin demand are reflected in changes in coin price, causing volatility and discouraging usage of coin as media-of-exchange.
Seigniorage shares~\cite{noteonshares}
argue that next-generation cryptocurrencies should incorporate an elastic supply rule that adjust the quantity of coin supply proportionately to changes in coin market value.

In a coin stabilisation scheme, changes in coin price stand proxy for changes in coin demand, and coin supply changes in response to changes in coin price. The idea is that an $X \%$ change in coin price, followed by an $X \%$ change in coin supply, will return coin price to its initial value, as as represented by the green box.

So the core operational principle of a protocol that aims to stabilise the market value of coin is the following rule: at the end of some pre-defined interval of time, if the change in coin price over the interval is $X \%$, change coin supply by $X \%$. More specifically, let's call that interval of time the rebase period, defined as every $n$ blocks. The coin supply rule mandates that:
$$
\begin{aligned}
Q_{i} &=Q_{i-1} \times \frac{P_{i}}{P_{i-1}} \\
\Delta_{i} &=Q_{i}-Q_{i-1}
\end{aligned}
$$
, where $i$ is the $\mathrm{i}-\mathrm{th}$ rebase period, $Q$ is coin supply and $P$ is coin price.

The solution to coin distribution offered, Seigniorage Shares, suggestS that there needs to be two types of coin: coin that acts like money and coin that acts like shares in the system's seigniorage.
For short, we'll just call these coins and shares. Coins and shares are identical in all respects (transaction verification works via ECDSA signature, etc) except for the process that regulates their respective supply.

Coins are the object of stabilisation, and $\Delta_{i}$ of coin is distributed to the holders of shares. When coin supply needs to increase, coinbase is distributed to share holders in exchange for a certain percentage of shares, which are destroyed (coin supply increases, share supply decreases). When coin supply needs to decrease, sharebase is distributed to coin holders in exchange for a certain percentage of coin, which are destroyed (coin supply decreases, share supply increases).

The mechanism of these shares-for-coin and coinfor-shares swaps is a voluntary one, a decentralised auction the rules of which are written into the protocol. The quantity of coins to create or destroy is defined via the $\Delta_{i}$ process in equations 3 and 4 , and there is an auction at the end of every rebase period.
When $\Delta_{i}$ is positive (new coins need to be created) a coin auction for $\Delta_{i}$ coins begins at the block or ledger set defining the start of rebase period $i+1$. Any holder of shares can bid for coins by signing and broadcasting a special TX describing the quantity of shares he is willing to trade for coin, and the minimum coins/shares price that he will accept. Winning bids are filled at whatever coins/shares price $P^{s}$ that clears the quantity to be sold. So $\Delta_{i}$ new coins are distributed to the winning bidders and $\Delta_{i} / P^{s}$ shares are destroyed. ${ }^{2}$

When $\Delta_{i}$ is negative (some existing coins need to be destroyed), a share auction of $\Delta_{i}$ worth of shares begins. Holders of coin can submit bids to purchase shares, signing a special TX describing the quantity of coins he is will to trade for shares, and the maximum coins/shares price $P^{s}$ that he will accept. Winning bids are filled at whatever price clears the quantity to be sold. So $\Delta_{i} / P^{s}$ new shares are distributed to the winning bidders and $\Delta_{i}$ coins are destroyed.

If the long-run demand for coin is positive, coin supply will increase with demand, but the quantity of shares will get increasingly scarce.






%1 讲一讲我理解的 $OHM 。首先说我非常看好项目。争议很多是因为超高APY看起来很像旁氏。但事实是这个“旁氏”越来越接近成功，尤其是经过519以及昨天的过山车考验之后。

%2 协议定位跟之前的算稳项目都不同，没有要求锚定1美元。这是一个非常聪明的决定，协议策略是首先吸纳足够多的资金(ProtocolControlledValue)，先壮大实力再去考虑其他目标。协议是backed, not pegged。

%3 $OHM 最成功的是引入了博弈论，对参与者来说越早参与获利越多，对于整个群体来说，所有都stake 是获利最大的解，这也是项目meme 3，3 的由来

%4 $OHM 的创新是通过出售bond的方式吸引更多资金锁定到PCV，用户通过bond获得折扣，协议通过bond锁定更多资金，属于双赢。这也反映了创始人 @ohmzeus的哲学： 拥有/购买流动性优于租赁流动性。
Ponzi, a design that old liability should be financed by issuing new debt,
Ponzi, a design that old liability should be financed by issuing new debt, has always been instinctively resented by the public.
Ponzi schemes,
where individuals or companies pay out funds to some parties by borrowing funds from others,


% Ponzi schemes normally share some common characteristics, and U.S. Securities and Exchange Commission~\cite{ponzi_gov} raises ``red flags'' for these warning signs, namely
% (1) high returns with little or no risk;
% (2) overly consistent returns;
% (3) unregistered investments;
% (4) unlicensed sellers;
% (5) secretive, complex strategies;
% (6) issues with paperwork;
% (7) difficulty receiving payments.
% Ponzi schemes are named after Charles Ponzi, who duped investors in the 1920s with a postage stamp speculation scheme.
% Ponzi scheme organizers often promise to invest your money and generate high returns with little or no risk.
% But in many Ponzi schemes, the fraudsters do not invest the money.
% Instead, they use it to pay those who invested earlier and may keep some for themselves.
% a Ponzi can be an investment fraud that pays existing investors with funds collected from new ones.
% where individuals or companies pay out funds to some parties by borrowing funds from others.

Fiat-collateralized stablecoins are pegged to the value of fiat, most often USD.
Fiat collateral remains in reserve with the central issuer and must reflect the number of corresponding stablecoins in circulation.
Collateralized: the stablecoin is a digital representation of the funds that collateralise it and every unit represents a claim on the issuer over the funds it receives from the users.
Crypto-collateralized: digital assets provide the backing rather that banks or cash using CDPs or collateralized debt positions.
Dai the first unbiased currency, over-collateralized
Frax, fractional-algorithmic stablecoin, being partially backed by collateral and partially stabilized algorithmically

Basis Cash~\cite{basiscash} is an Algorithmic Stablecoin
Pegged to 1 USD.
The protocol is designed to expand and contract supply similar to the way central banks trade fiscal debt to stabilize purchasing power, without any rebases or collateral risk.

Although there exists a wide variety of stablecoin mechanisms, Basis Cash specifically uses an “algorithmic central bank” approach to manage the supply of tokens according to a predetermined logic. The algorithm is in charge of balancing stablecoin supply to fluctuating demand, ensuring that the token price remains relatively stable.

There are three tokens in the Basis Cash design.
BAC - Basis Cash.
Basis Cash tokens are designed to be used as a medium of exchange. The built-in stability mechanism expands and contracts their supply, maintaining their peg to the MakerDAO Multi-Collateral Dai token (which roughly trades near the United States Dollar).

BAB - Basis Bonds.
Basis Bonds are minted and redeemed to incentivize changes in the Basis Cash supply. Bonds are always on sale to Basis Cash holders, although purchases are expected to be made at a price below 1 Basis Cash. At any given time, holders are able to exchange their bonds to Basis Cash tokens in the Basis Cash Treasury. Upon redemption, they are able to convert 1 Basis Bond to 1 Basis Cash, earning them a premium on their previous bond purchases.
Contrary to Basis Bonds of basis.io, bonds in Basis Cash do not have expiration dates. All holders are able to convert their bonds to Basis Cash tokens, as long as the Treasury has a positive BAC balance.

BAS - Basis Shares.
Basis Shares loosely represent the value of the Basis Cash network. Increased demand for Basis Cash results in new Basis Cash tokens to be minted and distributed to Basis Share holders, provided that the Treasury is sufficiently full.
Holders of Basis Share tokens can claim a pro-rata share of Basis Cash tokens accumulated to the Boardroom contract.

Tokens Distributed through
Yield Farming.
BAC and BAS tokens are distributed fairly through yield farming. Providing liquidity to BAC-DAI and BAS-DAI pairs result in additional BAS tokens being distributed.
This not only allows us to maintain our censorship resistance, but also acts as an incentive mechanism against lack of liquidity and bond death spirals — as famously pointed out with the original Basis.

When the price is above \$1
Basis Cash supply is expanded to bring the price back down. The ones who staked Basis Shares on the Boardroom will receive BAC seigniorage as rewards.
When the price is below \$1
The protocol auctions off Basis Bonds for BAC to contract Basis Cash supply. They can be redeemed for premiums after BAC price returns to its 1 dollar peg.

==> [CryptEx23] Rational Ponzi Game in Algorithmic Stablecoin/table/stablecoins.tex <==
\begin{table}[!hbt]
\renewcommand\arraystretch{1.2}
\caption{An Overview of Stablecoins (Ranked by Market Cap)}
% \scriptsize
\label{tab:stablecoin}
\begin{center}
\resizebox{0.97\linewidth}{!}{
\begin{tabular}{l|l l l l r r}
\toprule
\textit{\textbf{Name}} &  \textit{\textbf{Token}} & \textit{\textbf{Centralised}}  & \textit{\textbf{Supply}} & \textit{\textbf{Peg}} & \textit{\textbf{Mrk Cap}}\\
\midrule

 \textbf{Tether}   &  USDT   & Centralised   &  Collateral   &  USD  &  \$157.4B    \\
 \textbf{USD Coin}   &  USDC   & Centralised   &  Collateral   &  USD  &  \$68.5B    \\
 \textbf{BinanceUSD}    & BUSD  & Centralised   &  Collateral   &  USD  &  \$21.5B    \\
 \textbf{Dai}   & DAI  & Decentralised  &  Collateral   &  USD  &  \$6.2B    \\
 \textbf{Frax}   & FRAX   &  Decentralised   &  Fractional Alg.  &  USD  &  \$1.4B    \\
 \cellcolor{pink} \textbf{TerraUSD}   & UST-LUNA  &  Decentralised    &  Alg. (S.Share) &  USD  &  \$471.1M   \\
 \textbf{Olympus}  & - & Decentralised  &  Collateral Alg.   &  USD  &  \$303.4M    \\ 
 \textbf{Fei USD}   & FEI  &  Decentralised   &  Collateral B.C.   &  USD  &  \$57.2M    \\
 \cellcolor{pink} \textbf{Ampleforth}   &  AMPL  & Decentralised  &  Alg. (Rebase)  &  CPI USD  &  \$45.6M    \\
 \textbf{Empty Set}   &  ESD   &  Decentralised   &  Alg. (S.Share)   &  USD  &  \$370.5K   \\
 \textbf{Basis Cash}  &  BAC-BAB-BAS   & Decentralised   &  Alg. (S.Share)   &  USD  &  \$281.7K   \\
 
%  \textbf{Tether}   &  USDT   & Centralized   &    &   &     \\
%  \textbf{USD Coin}   &  USDC    & Centralized     &  Fair-CS &    & Centralized &   &   \\  
%  \textbf{BinanceUSD}    & BUSD  & Centralized   &     &   \\  
%  \textbf{Dai}   & DAI   &  Decentralized     &  Over-CS & Decentralized  &   &   \\
%  \textbf{Fei USD}   & FEI   &  Decentralized    & Over-CS  & PCV, bonding curve &  &   &    \\
%  \textbf{Ampleforth}   &  AMPL  &  Decentralized   &    AS & - & Elastic supply (rebase) & AMPL &   & \\
%  \textbf{Empty Set}   &  ESD   &  Decentralized    &   AS  & - & introduce bond  &   &    \\
%  \textbf{Basis Cash}  &  BAC-BAB-BAS  &  Decentralized    & AS & - & introduce share and bond & BAC-BAS-BAB & peg to 1  &   &   \\
%  \textbf{Frax}   & FRAX   &  Decentralized   &  fractional-AS  & & burn and redeem & FRAX-FXS & peg to 1 &   &   \\
%  \textbf{TerraUSD}   & UST-LUNA  &  -   & AS  & &  burn and redeem & Luna-UST & peg to 1 & 50B USD  &   &   \\
%  \textbf{Olympus}   & OHM  &  Decentralized  &  (3,3) POL &  NO & peg to 1  & \$303m  &   &   \\

\bottomrule
\end{tabular}
}
\begin{tablenotes}
       \footnotesize
       \item[] 
        \textbf{Update:} Data fetched on 12th Oct, 2022. \textbf{Abbreviation:} Alg. = Algorithmic;
       \item[]  
        S.Share = Seigniorage Shares; B.C. = Bonding Curve; Mrk = Market.
\end{tablenotes}
\end{center}
\vspace{-0.5cm}
\end{table}


==> table/stablecoins.tex <==
\begin{table}[!hbt]
\renewcommand\arraystretch{1.2}
\caption{An Overview of Stablecoins (Ranked by Market Cap)}
% \scriptsize
\label{tab:stablecoin}
\begin{center}
\resizebox{0.97\linewidth}{!}{
\begin{tabular}{l|l l l l r r}
\toprule
\textit{\textbf{Name}} &  \textit{\textbf{Token}} & \textit{\textbf{Centralised}}  & \textit{\textbf{Supply}} & \textit{\textbf{Peg}} & \textit{\textbf{Mrk Cap}}\\
\midrule

 \textbf{Tether}   &  USDT   & Centralised   &  Collateral   &  USD  &  \$157.4B    \\
 \textbf{USD Coin}   &  USDC   & Centralised   &  Collateral   &  USD  &  \$68.5B    \\
 \textbf{BinanceUSD}    & BUSD  & Centralised   &  Collateral   &  USD  &  \$21.5B    \\
 \textbf{Dai}   & DAI  & Decentralised  &  Collateral   &  USD  &  \$6.2B    \\
 \textbf{Frax}   & FRAX   &  Decentralised   &  Fractional Alg.  &  USD  &  \$1.4B    \\
 \cellcolor{pink} \textbf{TerraUSD}   & UST-LUNA  &  Decentralised    &  Alg. (S.Share) &  USD  &  \$471.1M   \\
 \textbf{Olympus}  & - & Decentralised  &  Collateral Alg.   &  USD  &  \$303.4M    \\ 
 \textbf{Fei USD}   & FEI  &  Decentralised   &  Collateral B.C.   &  USD  &  \$57.2M    \\
 \cellcolor{pink} \textbf{Ampleforth}   &  AMPL  & Decentralised  &  Alg. (Rebase)  &  CPI USD  &  \$45.6M    \\
 \textbf{Empty Set}   &  ESD   &  Decentralised   &  Alg. (S.Share)   &  USD  &  \$370.5K   \\
 \textbf{Basis Cash}  &  BAC-BAB-BAS   & Decentralised   &  Alg. (S.Share)   &  USD  &  \$281.7K   \\
 
%  \textbf{Tether}   &  USDT   & Centralized   &    &   &     \\
%  \textbf{USD Coin}   &  USDC    & Centralized     &  Fair-CS &    & Centralized &   &   \\  
%  \textbf{BinanceUSD}    & BUSD  & Centralized   &     &   \\  
%  \textbf{Dai}   & DAI   &  Decentralized     &  Over-CS & Decentralized  &   &   \\
%  \textbf{Fei USD}   & FEI   &  Decentralized    & Over-CS  & PCV, bonding curve &  &   &    \\
%  \textbf{Ampleforth}   &  AMPL  &  Decentralized   &    AS & - & Elastic supply (rebase) & AMPL &   & \\
%  \textbf{Empty Set}   &  ESD   &  Decentralized    &   AS  & - & introduce bond  &   &    \\
%  \textbf{Basis Cash}  &  BAC-BAB-BAS  &  Decentralized    & AS & - & introduce share and bond & BAC-BAS-BAB & peg to 1  &   &   \\
%  \textbf{Frax}   & FRAX   &  Decentralized   &  fractional-AS  & & burn and redeem & FRAX-FXS & peg to 1 &   &   \\
%  \textbf{TerraUSD}   & UST-LUNA  &  -   & AS  & &  burn and redeem & Luna-UST & peg to 1 & 50B USD  &   &   \\
%  \textbf{Olympus}   & OHM  &  Decentralized  &  (3,3) POL &  NO & peg to 1  & \$303m  &   &   \\

\bottomrule
\end{tabular}
}
\begin{tablenotes}
       \footnotesize
       \item[] 
        \textbf{Update:} Data fetched on 12th Oct, 2022. \textbf{Abbreviation:} Alg. = Algorithmic;
       \item[]  
        S.Share = Seigniorage Shares; B.C. = Bonding Curve; Mrk = Market.
\end{tablenotes}
\end{center}
\vspace{-0.5cm}
\end{table}

